Evolve Together, Fall into Place: How Social Scaffolding Shapes Self-Evolving Multi-Agent Systems

Recent work lets LLM agents evolve their own harness, up to the team itself. Yet in human groups, the same abilities achieve different outcomes under different social conditions. Borrowing the notion of scaffolding from developmental psychology, we investigate whether the social scaffolding of a self-evolving multi-agent system (MAS), namely its team composition and structure of interdependence (e.g., collaboration, conformity, or competition), shapes how the team evolves. We present AGORA (Agents Growing through Organization and Relational Arrangements), a framework that varies the two axes independently across three evolution mechanisms. Across web search, codebase understanding, and document QA, we find that (1) evolution alone rarely helps, while the right scaffolding surpasses a strong agent evolved alone by up to 25 points; (2) it does so by moving authority to the most capable member while the others step back; and (3) this member, having grown within the team, outperforms the same model alone. Designing a self-evolving MAS thus requires designing its social scaffolding, which shapes not only how its agents learn, but who gets to lead.

==> latex/table/tab_composition.tex <==
\begin{table*}[t]
\centering

\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
Benchmark & Chairman & Other roles & Strong roles in \textit{weakstrong} \\
\midrule
GAIA & plan\_agent & web\_agent, file\_agent, answer\_agent & web\_agent \\
LoCoBench & planner & developer, reader-1--4 & developer \\
OfficeQA & planner & reader-1, reader-2, calculator, answer\_agent & reader-1, reader-2 \\
\bottomrule
\end{tabular}
}

\vspace{4pt}

\resizebox{\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
Team & Agents & Model assignment \\
\midrule
solo & One agent with all tools of the benchmark & All weak / all strong \\
onlyweak & Full MAS & All weak \\
weakstrong & Full MAS & One bottleneck role strong (all its instances), the rest weak \\
onlystrong & Full MAS & All strong \\
\bottomrule
\end{tabular}
}

\caption{Team compositions. Top: roles per benchmark. Bottom: model assignment per team type. Weak: Qwen3-30B-A3B-Instruct-2507; strong: Qwen3.6-35B-A3B.}
\label{tab:composition}
\end{table*}

